Who should I trust? A Visual Analytics Approach for Comparing Net Load Forecasting Models

Net load forecasting is crucial for energy planning and facilitating informed decision-making regarding trade and load distributions. However, evaluating forecasting models' performance against benchmark models remains challenging, thereby impeding experts' trust in the model's performance. In this context, there is a demand for technological interventions that allow scientists to compare models across various timeframes and solar penetration levels. This paper introduces a visual analytics-based application designed to compare the performance of deep-learning-based net load forecasting models with other models for probabilistic net load forecasting. This application employs carefully selected visual analytic interventions, enabling users to discern differences in model performance across different solar penetration levels, dataset resolutions, and hours of the day over multiple months. We also present observations made using our application through a case study, demonstrating the effectiveness of visualizations in aiding scientists in making informed decisions and enhancing trust in net load forecasting models.

==> sections/old/introduction.tex <==
\section{Introduction}
\kaustav{In Progress}The net-load of an electric grid can be defined as the difference between the total electricity demand and the electricity generation from behind-the-meter resources such as solar and other distributed generators~\cite{NetLoadDefinition}. It can vary based on various factors, including weather conditions and the time of the day. Understanding net-load is of paramount importance in energy planning and management. Accurate net-load forecasting enables grid operators, policymakers, and energy providers to make informed decisions regarding energy trade, load distribution, and resource allocation. By accurately predicting the net-load, the stakeholders can optimize the operation of power plants, plan for future infrastructure upgrades, and ensure a stable and reliable electricity supply. However, the proliferation of solar energy generation sources in residential settings has significantly impacted the performance of traditional net-load forecasting models~\cite{SolarEnergyPenetration}.

\kaustav{add more of trust here}This necessitates the development of time-series forecasting methods that can reliably predict the net-load and quantify its uncertainty and variability across different time periods and solar penetration levels. We have collaborated with scientists who have developed a deep-learning model that generates probabilistic forecasts for net-load across different solar penetration levels and prediction horizons~\cite{sen2022kpf}. Leveraging various input variables like temperature, humidity,  apparent power, solar irradiance, etc., this model generates day-ahead net-load predictions at a 15-min time resolution. Notably, it shows superior performance against existing benchmarks and also demonstrates robustness against missing input values.

However, in order to improve trust in the model, these outputs need to be explored by domain experts, including scientists and grid operators. The model's performance may fluctuate due to seasonal variations in the input variables, and stakeholders must also assess its reliability in the face of noisy inputs mirroring real-life scenarios. Nevertheless, this process can be complex and time-consuming for busy grid operators. Hence, a visual analytic approach that can perform these tasks to improve trust in the model's performance is the need of the hour.

In light of this, we collaborated with energy scientists to thoroughly investigate the model's performance across diverse time periods and input scenarios, gaining valuable insights into the evaluation tasks needed to comprehend its effectiveness. Building upon this experience, we performed a design study to develop a comprehensive system aimed at facilitating stakeholders in performing these evaluation tasks in an efficient manner. As a result, we developed a visual analytics framework that empowers users to gain an in-depth understanding of the model's performance, effectively leveraging data visualization techniques to aid informed decision-making in the realm of energy planning and grid operations.

Our proposed framework aims to provide a comprehensive understanding of various aspects related to net load forecasting. Firstly, it enables scientists to assess net load variability concerning input variables by comparing model forecasts with actual net load values across different time periods and seasons. By analyzing the effects of variables like temperature, humidity, and apparent power on net-load forecasts, users can gain insights into their impact on the model's performance. 
Secondly, the framework facilitates an in-depth forecast error analysis, comparing the model's forecast errors with respect to different input variables. Users can examine the relationships between forecast errors and input variables in various scenarios, including outlier removal, error rate assessment at different granularity levels, and the implementation of time shifts to understand the influence of input variables at different points in time. Furthermore, the framework includes evaluating forecast errors with noisy inputs at different noise levels, thus providing information for improving the model's reliability and robustness in real-world scenarios. Our comprehensive visual analytic framework can empower scientists and grid operators to make data-driven decisions, enhancing trust and confidence in the net load forecasting model.

Our approach represents a distinct and valuable contribution to the field of net load forecasting. While prior research has primarily concentrated on developing interfaces during the model development process, tailored to aid model developers, our focus lies in the post-hoc evaluation of the model's performance, catering specifically to the needs of energy scientists and grid operators~\cite{lucas2021lumen, klaus2023visual}. There are other works that explore the performance of probabilistic net-load forecasting models through different visualization charts but do not offer an integrated interactive interface~\cite{wang2017data, henriksen2022electrical}. Our framework presents an integrated workflow that empowers users to explore net load variability and forecast error analysis concerning various input variables and scenarios, which makes it a novel approach in this domain. Furthermore, previous research has demonstrated that visual analytic methods can significantly enhance trust in model outputs during complex sense-making tasks, thereby providing further validation for the efficacy of our approach~\cite{dasgupta2016familiarity}.

\aritra{review criteria for us to remember: 1. Evidence of actual deployment or application
2. Representative of a state-of-the-art capability or practice
3. Ability to inform strategies for advancing grid capabilities}\kaustav{Sure}
